From Web(logs) to Web(AI): Questions, Platforms, and Methods across Twenty Editions of ICWSM

Over twenty editions, the ICWSM community has examined social life online as platforms, interactions, and research methods have changed. What can this body of research tell us at this critical juncture, as AI increasingly reshapes how people communicate online? We analyzed 2,139 indexed contributions from 2007 to 2026, distinguishing topics identified through nonnegative matrix factorization from problem framings captured through explicit textual cues. We find that platform mentions shift from blogs toward Twitter and, more recently, Reddit. Online community research maintains a similar topic share (10.5% to 10.0%), but governance cues within it increase from 4.0% to 34.3%. Harm-related cues also increase after restricting abstracts to a fixed length. Our review also traces advances in sampling, measurement, and causal and experimental methods. We discuss how AI-mediated interactions complicate these questions and provide a reporting checklist to support research across changing platforms.

==> 01_introduction.tex <==
% !TeX root = 0paperICWSM.tex
\section{Introduction}
Social media offers opportunities to study self-expression, relationships, support, and public participation. Since 2007, the International AAAI Conference on Web(logs) and Social Media (ICWSM) has examined these activities and the methods used to understand them. 
The first ICWSM, in 2007, studied weblogs. 
Blogs appear in 35.2\% of contributions from the conference's first five editions and in 0.9\% of contributions from its most recent five. By 2015, the conference had dropped ``Weblogs'' from its name while keeping its acronym. Twitter then rose to 45.7\% of contributions in 2012--2016 and fell to 24.8\% in 2022--2026. Each shift raises the same question: does research on an earlier platform still describe how people interact online? As AI systems increasingly rank, rewrite, generate, and moderate online interaction \citep{hancock2020,hohenstein2023}, the field faces a sharper version of that question: is social media still the right object of study, or have its central questions moved to AI?

ICWSM's twentieth edition offers a record of what survives these shifts. We separate the subjects the conference studied from the problems researchers asked about them, then trace methodological questions across platform contexts.

Topics alone cannot capture this history. Researchers can study the same subject while pursuing different questions. Community research can examine how participation develops, how members provide support, or how rules are enforced. Methods also shape what can be learned. Studies have evaluated Twitter sampling \citep{p14401}, tested adjustments for textual confounding \citep{p19362}, and used randomized prompts or quasi-random server assignment to study communication \citep{p19308,p31365}. Following subjects, problem framings, and forms of evidence together gives a fuller account of the field.

We build on computational histories of research communities \citep{hall2008,liu2014,wallace2017} and the reflective approach of the FAccT retrospective \citep{facct2022}. Within ICWSM, work on geographical representation shows why diversity of subjects or platforms cannot stand in for diversity of populations studied \citep{weird2024}. We ask:
\begin{itemize}
\item \textbf{RQ1:} How have ICWSM's topics and platform contexts evolved across editions?
\item \textbf{RQ2:} How have problem framings changed across and within research topics?
\item \textbf{RQ3:} How do selected studies illustrate methodological developments and recurring challenges across changing platform contexts?
\end{itemize}

We analyze titles and abstracts from 2,139 indexed contributions across 2007--2026. We distinguish topics, or the subjects and tasks represented in scholarly text, from problem framings, or the questions and concerns expressed within those subjects. Topic modeling describes the former; framing cues approximate the latter. Four fixed five-edition periods provide a common basis for comparison. Selected literature supplies context for interpreting methods without estimating their adoption across the conference.

We find topical continuity alongside changing problem framing. The community component remains near one tenth of the topic mixture, while governance-related framing becomes much more common. The contrast persists when we remove governance features from the topic representation and restrict abstracts to a fixed length. Harm-related cues also rise under fixed-length checks.

This paper contributes a documented corpus of twenty ICWSM editions with longitudinal topic, framing, and platform measures. We separate topic change from changes in problem framing, using community research and governance as a detailed case. We also synthesize recurring methodological problems across platform contexts and turn them into a reporting checklist for AI-mediated interaction. We will release the corpus and analysis materials upon publication. 
% Platforms change; the questions recur.


==> 06_research_agenda.tex <==
% !TeX root = 0paperICWSM.tex
\section{Discussion}
Two decades of ICWSM show substantial platform turnover without erasing familiar research problems. Community research makes this visible: its topic share changes little across the endpoint periods, while governance cues become much more common. The literature shows why that distinction matters. Sampling still determines whose behavior enters a study; traces still need construct validation; causal claims still depend on comparison design; moderation still embeds judgment; and data access still constrains what researchers can observe. AI changes each of these conditions, especially the provenance of language and exposure.

\paragraph{Following questions within topics.}
Topical continuity can conceal changes in what researchers seek to explain or improve. Retrospectives can connect subjects with research questions, designs, and intended beneficiaries. The weak stability of our phase boundaries favors overlapping interests over sharply separated eras. Historical interviews and archival work could explain changes that publication profiles cannot.

\paragraph{Making methodological comparisons reusable.}
Table~\ref{tab:checklist} turns recurring design questions into reporting items. A later reader should be able to judge whether a finding still applies after a platform, access regime, or content-production process changes. The checklist is a reporting aid; it does not certify that an assumption holds.

\input{tables/reporting_checklist}

\paragraph{Interpreting AI-mediated interaction.}
AI-mediated communication includes systems that modify, augment, or generate messages on a person's behalf \citep{hancock2020}. A post can now reflect a person's intentions, model suggestions, interface defaults, and platform rules. Final text alone may no longer reveal who composed a message or whose attention it represents.

This matters for measures that infer attitudes, distress, or social support from text. Experiments with suggested replies show that assistance can change language and interpersonal evaluations, while suspected assistance can lower how a partner is perceived \citep{hohenstein2023}. Language quality, perceived care, and interaction benefit should be measured separately. Our LLM-related publication counts motivate these questions; they do not measure how much social media communication is AI-mediated.

AI mediation also changes exposure. A person may encounter generated replies, ranking decisions, and moderation actions that change over time. Studies can record whether people composed, edited, selected, or only received generated content, together with system versions and interaction context. Consented process records, participant accounts, and interface experiments can provide evidence that final text cannot recover. These records support questions about delegation, trust, social obligation, and community norms even when human and machine contributions cannot be cleanly separated.

\paragraph{Preserving comparisons across changing systems.}
Platform access, model versions, and content-production processes can change both behavior and observation. Recording validation evidence, disagreement, collection conditions, and system versions lets later researchers assess whether an earlier finding transfers. Cumulative comparisons depend on preserving the conditions under which a claim was supported.


==> checklist.tex <==
\section*{Paper Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes. The study analyzes public scholarly publications and metadata. It involves no new participants and no analysis of individuals' social media posts (see Ethical Considerations).}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes. The abstract and introduction describe topics and problem-framing cues at the scope supported by the analysis, and Section~3 states that the methodological examples are illustrative.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made?
    \answerYes{Yes. Section~3 explains what topic mixtures and framing cues measure, their limitations, the sensitivity analyses, and how the literature examples were selected. Appendices~B and C provide the topic terms and framing codebook.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
   \answerYes{Yes. We examine abstract length, historical vocabulary, shared vocabulary between topics and framing cues, platform composition, paper composition across editions, and corpus coverage (Sections~3, 4, and 7; Appendix~D).}
    % \answerYes{Yes. We examine abstract length, historical vocabulary, shared vocabulary between topics and framing cues, paper composition across editions, and corpus coverage (Sections~3, 4, and 7; Appendix~D).}
  \item Did you describe the limitations of your work?
    \answerYes{Yes. See Section~7.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes. Publication counts and textual cues could be misread as indicators of research quality or community concern (see Ethical Considerations).}
  \item Did you discuss any potential misuse of your work?
    \answerYes{Yes. We caution against using the measures to rank researchers or judge research quality (see Ethical Considerations).}
  \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes. We provide explicit measurement definitions, sensitivity analyses, a codebook, and an independent validation protocol, and we document provenance and reuse constraints for the planned release (Section~3; Appendices~C, D, and F; Ethical Considerations). We do not infer sensitive attributes of authors.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA. The study is descriptive and does not test hypotheses or develop theoretical results.}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA.}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA.}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA. We nevertheless examine measurement-based alternative explanations for the observed patterns, including abstract length and shared vocabulary (Section~3; Appendix~D).}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA.}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA.}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA.}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA.}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{NA.}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{No. The corpus, derived measurements, analysis code, and documentation will be released upon publication; no anonymous release is included with this review submission.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes. Section~3 reports the TF--IDF representation, vocabulary threshold, number of components, initialization, random seed, iteration limit, and alternative specifications. The unsupervised analysis uses no data splits.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes. We report 95\% within-edition resampling intervals from 2,000 resamples (Sections~3 and 4; Figures~1--3) and compare alternative component counts and random initializations.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{No. Hardware-specific resources and total compute were not recorded.}
  \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made?
    \answerYes{Yes. Sections~3 and 7 state which claims the current evidence supports and which require independent validation. Appendix~F specifies that validation protocol.}
  \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerYes{Yes. We discuss how incidental cue matches and missed concerns affect interpretation of prevalence estimates (Sections~3, 4, and 7; Appendix~C) and how the measures could be misread as quality indicators (Ethical Considerations).}
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes. We cite Crossref, the AAAI proceedings archive, the official ICWSM 2007 program, and the publications discussed in the paper.}
  \item Did you mention the license of the assets?
    \answerYes{Yes. Crossref bibliographic metadata is reusable without restriction, while abstracts remain subject to publisher or author copyright. We therefore do not plan to redistribute source papers or bulk abstracts (see Ethical Considerations).}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNo{No. The corpus, derived measurements, analysis code, and documentation will be released upon publication.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes. The study uses published scholarly metadata and involves no human participants. No additional consent was obtained, and author names are retained only for bibliographic attribution (see Ethical Considerations).}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes. The only personal information is author names in bibliographic records. We do not infer sensitive attributes or rank researchers (see Ethical Considerations).}
  \item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
    \answerYes{Yes. The planned release will use persistent identifiers, source links, machine-readable derived measurements, documented inclusion decisions, and provenance and reuse documentation (see Ethical Considerations).}
  \item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})?
    \answerNo{No. A data card will accompany the release upon publication.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{NA. The reported analyses involve no participants. Appendix~F specifies a future independent coding protocol; its results are not reported in this paper.}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{NA.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{NA.}
  \item Did you discuss how data is stored, shared, and deidentified?
    \answerNA{NA.}
\end{enumerate}

\end{enumerate}

